Modeling and Leveraging Prerequisite Context in Recommendation

Prerequisites can play a crucial role in users' decision-making yet recommendation systems have not fully utilized such contextual background knowledge. Traditional recommendation systems (RS) mostly enrich user-item interactions where the context consists of static user profiles and item descriptions, ignoring the contextual logic and constraints that underlie them. For example, an RS may recommend an item on the condition that the user has interacted with another item as its prerequisite. Modeling prerequisite context from conceptual side information can overcome this weakness. We propose Prerequisite Driven Recommendation (PDR), a generic context-aware framework where prerequisite context is explicitly modeled to facilitate recommendation. We first design a Prerequisite Knowledge Linking (PKL) algorithm, to curate datasets facilitating PDR research. Employing it, we build a 75k+ high-quality prerequisite concept dataset which spans three domains. We then contribute PDRS, a neural instantiation of PDR. By jointly optimizing both the prerequisite learning and recommendation tasks through multi-layer perceptrons, we find PDRS consistently outperforms baseline models in all three domains, by an average margin of 7.41%. Importantly, PDRS performs especially well in cold-start scenarios with improvements of up to 17.65%.

==> review/comments.tex <==
**Overall Concerns**

From Education perspective,

- Lack of the technology-enhanced learning context
> HC: ignore
- poor match of data and approach: two of the datasets do not match the knowledge acquisition/learning-scenario addressed in the paper
> HC: ignore
- related work: the approach should position itself better in the context of learning-related recommender systems (an active research area since many years that is often lacking a grounding the actual RecSys state-of-the-art)

From RS perspective,

- there is also a wealth of further baselines with which to compare
HC: accept, but ignore
- Lack of some import details
    - it is unclear if the in prerequisite knowledge mining stage included test data (data leakage)
    > HC: accept. TODO: distinguish the two stage more clearly
    - There are 2 splitting: prior, target, normally-used data; train, test, validation data. It’s not clear of the usage of them.
    > HC: re-stated them in section 3 and section 5.
- Assumption:
    - Re-think about the assumption that “users have mastered the knowledge contained in items previously interacted with”.
    - The prior and target knowledge states do not change during the remaining interaction sequence, which is not realistic.
    - After the proposed recommender is deployed, interactions corresponding to the target knowledge cannot be obtained in this manner. This is because we only have interaction data before the target time point in that situation.
- RW: The paper overlooks several lines of relevant research.
    - Sequential Recommendation. (the meaning of the prerequisite is unclear)
    - Progression modeling to capture the transitions of user interests
    - Knowledge tracing
- Approach
    - The details are not clear enough.
        - E.g., what is a fully-connected graph? How is it constructed? Is it different from the graph used for applying TextRank in the previous step? These may be explained in the literature [24], but I think the description should be self-contained as this part is a core process of the proposed solution.
        HC: accepted, but nore sure how to state it in a short space.
        - Wikipedia Reference Distance: It is unclear to me how the authors find Wikipedia concepts (equivalent to articles?) related to a given concept.
    - Annotation: How did you select 300 samples? Who annotated those samples? What are annotation criteria? How consistent were the annotations provided by different people?
    - The proposed method is less sophisticated
        - MLPs is rather naive compared to recent recommenders.
        - Is simply averaging knowledge embeddings sufficient for this task?
- Dataset
    - Consider using Knowledge Tracing Datasets?
- Evaluation
    - Negative sampling is reported to be a bad practice making evaluation results unreliable.
    - Consider adding sequential recommenders as baselines.
- Result
    - It’s not able to judge the accuracy of the statement “We also find that prerequisite graphs have different structural properties”.
    - Cold-start: It is unclear to me how the authors obtained the embeddings for users and items unseen in the training phase.
    > HC: it's randomly initialized. I think it is not necessary to state.

**Minor Concerns**

- How did we arrive at the 30% and 20% splitting ratios?
- Who annotated what and with what inter-rater agreement?
- It’s not transparent that how the two prerequisite metrics are considered in the model.
- Until reading Section 5.1, I did not understand what item documents are. (Re-structure this description.)
> HC: accepted, mentioned what documents is in section 3.
- KLP and KPL make confusion.
> HC: accepted.
- Equation 1: Is $\sigma$ the sigmoid function?
> HC: solved.
- Section 5.1, `500 labeled samples`: According to Section 3, there are 300 annotated samples.
> HC: solved. 300
- Section 6.1: There is a reference error.
> HC: solved
- Figure 4 is not referred in text.
> HC: solved

==> review/slide.tex <==
%%%%%%%%%%%%%%%%%%%%% Page 1 %%%%%%%%%%%%%%%%%%%%%
[Title + Name + Affiliation]


%%%%%%%%%%%%%%%%%%%%% Page 2 %%%%%%%%%%%%%%%%%%%%%
[Introduction]
“it is also important to incorporate the contextual information into the recommendation process in order to recommend items to users under certain circumstances”
				---- From RS Handbook (2022)

For example,
Such circumstance can be temporal information, or location that independent with users or items, but can be reflected from their interaction records in some way.
(Context, User) => item
(Winter, The User Interacted with Sporting Equipment) => Skiting Shoses
Common sense: Winter usually has snow

Prerequisite is also a certain kind of knowledge circumstance that constrains user’s action.
- Context: The stage of an primitive/advanced level of knowledge
- User: mostly interacted with statistic-based course
- Common sense: the prerequisite relation of knowledge, .e.g, Naïve Bayes is the pre-conditional constrain of Bayes Classifier.
% For example, using the temporal context, a travel recommender system would provide a vacation recommendation in the winter that can be very different from the one in the summer. Similarly, in case of personalized content delivery on a website, a user might prefer to read world news when she logs on the website in the morning and the stock market report in the evening, and on weekends to read movie reviews and do shopping, and appropriate recommendations should be provided to her in these different contexts.

%%%%%%%%%%%%%%%%%%%%% Page 3 %%%%%%%%%%%%%%%%%%%%%
[Introduction]
Prerequisite is a term that usually used in Educational-related Domain.

Prerequisite is a certain kind of knowledge circumstance that constrains user’s action.
- If a person do not have the knowledge about Bayes, then we should not recommend Bayes Classifier to him/her.


%%%%%%%%%%%%%%%%%%%%% Page 4 %%%%%%%%%%%%%%%%%%%%%
[Introduction]
> Why prerequisite is helpful (for recommender)?
    : A case

%%%%%%%%%%%%%%%%%%%%% Page 5 %%%%%%%%%%%%%%%%%%%%%
[Problem Definition]
> To align with the general CARS, our PDRS is formulated as ..


%%%%%%%%%%%%%%%%%%%%% Page 6 %%%%%%%%%%%%%%%%%%%%%
[Data Construction]
> Keyword extraction.


%%%%%%%%%%%%%%%%%%%%% Page 7 %%%%%%%%%%%%%%%%%%%%%
[Data Construction]
> 2 branches to build such inference unbalance.


%%%%%%%%%%%%%%%%%%%%% Page 8 %%%%%%%%%%%%%%%%%%%%%
[Approach]
> Two-tower MLP


%%%%%%%%%%%%%%%%%%%%% Page 9 %%%%%%%%%%%%%%%%%%%%%
[Experiment]
Main Results + Ablation


%%%%%%%%%%%%%%%%%%%%% Page 10 %%%%%%%%%%%%%%%%%%%%%
[Discussion 1,2,3,4]



==> sec/note.tex <==
\section{Note}
Include Yet:
\begin{itemize}
    \item Originally, we highlighted that the model is SOTA -> Currently, I'm telling the story as a wrok to full-fill the research gap. Because I find my proposed model can not beat the KGCN, on of the KG-RS SOTA, constructing a lot KG message process and is more elegant at handling KG. Thus, our main contribution lies in introducing prerequisite, a special kind of knowledge, into RS, rather than letting RS become a SOTA model by using additional information.
    Regarding this, I've updated Abs/Intro/Approach
    \item I changed Preliminary(Original) to a re-definition of this problem, i.e. we define a new type of problem -- i.e., PDR problem aiming to recommend the ideal item to user logically. And our model, that is PDRS, is just an instantiation of the task. Regarding this, I've updated PDR Task.
    \item Regarding the insufficient discussion of prerequisite, I have included a separate study of the prerequisite role in the discussion, adding RQ2 to discuss how prerequisite approachable to downstream RS. Regarding this, I've updated PDR Task.

\end{itemize}

Not Include Yet, And Doubt Whether to Include Them:
\begin{itemize}
    \item Compared to normal KG, What is the superiority of PG (Prerequisite Graph)?
    From Liangming: KG is a general objective knowledge, but PG has some guidance for RS, it is a subjective one.
    
    \item To mention the sequential recommender somewhere as a future work.
    \item Related Work is not close enough to the new story.
\end{itemize}


Story from liangming:
\begin{itemize}
    \item The drawbacks of noraml CF -> Why commonsense knowledge is needed -> Exsisting work -> Gap: they are focusing on normal KG -> the drawbacks of normal KG [?] -> Gap: Prerequisite Graph is more appropriate for recommendation, and it is neglected -> PG v.s. KG (Giving examples) -> Purpose
\end{itemize}
